Establishing Baselines for Photonic Quantum Machine Learning: Insights from an Open, Collaborative Initiative

The Perceval Challenge is an open, reproducible benchmark designed to assess the potential of photonic quantum computing for machine learning. Focusing on a reduced and hardware-feasible version of the MNIST digit classification task or near-term photonic processors, it offers a concrete framework to evaluate how photonic quantum circuits learn and generalize from limited data. Conducted over more than three months, the challenge attracted 64 teams worldwide in its first phase. After an initial selection, 11 finalist teams were granted access to GPU resources for large-scale simulation and photonic hardware execution through cloud service. The results establish the first unified baseline of photonic machine-learning performance, revealing complementary strengths between variational, hardware-native, and hybrid approaches. This challenge also underscores the importance of open, reproducible experimentation and interdisciplinary collaboration, highlighting how shared benchmarks can accelerate progress in quantum-enhanced learning. All implementations are publicly available in a single shared repository (https://github.com/Quandela/HybridAIQuantum-Challenge), supporting transparent benchmarking and cumulative research. Beyond this specific task, the Perceval Challenge illustrates how systematic, collaborative experimentation can map the current landscape of photonic quantum machine learning and pave the way toward hybrid, quantum-augmented AI workflows.

==> participants_sections/Qubiteers/old_results.tex <==
\begin{itemize}

\item[1.] \textbf{Validation Accuracy:} \
We compare the classification performance of all models on the MNIST dataset using both 5-channel and 20-channel PQK embeddings. Table~\ref{tab:acc5} summarize the validation and training accuracies. Notably, the hybrid model using Type~1 PQK with 20 output channels achieves a 1.4\% improvement in validation accuracy over the classical baseline.

\begin{table}[h]
\centering
\label{tab:acc5}
\begin{tabular}{lccc}
\toprule
Model & Quantum Encoding & Val Accuracy (\%) & Train Accuracy (\%) \\
\midrule
Full Baseline CNN (no quantum) & None & 97.1 & 99.5 \\
Quantum-augmented Baseline CNN & None & 97.5 & 99.6 \\
Hybrid CNN + PQK (Static) & Type~1 (5 ch) & 98.5 & 99.9 \\
Hybrid CNN + PQK (Static) & Type~2 (5 ch) & \verb|~|10 & 79.9 \\

% Hybrid CNN + PQK (with Merlin) & Type~2 (Trainable) () & 96.0 & 99.8 \\

% Hybrid CNN + PQK (Trainable) & Type~2  ((3x3)$\rightarrow$(5x5)) & 96.0 & 98.0\% \\
Hybrid CNN + PQK (Trainable) & Type~2  (2 PQK Layers) & 96.0 & 98.0\% \\

Hybrid CNN + PQK (Trainable) & Type~2  (1 PQK Layer) & 97.0 & 98.8\% \\

% One convolution layer of Type 2 PQK, with kernel size 3 & 10 & $\approx$ 98.0\% \\
CNN-PQK Parallel & Type~2 (2 PQK Layers) & $\approx$ 95.2\% & 97.7\% \\
\bottomrule
\end{tabular}
\caption{Validation accuracy on MNIST (in \%) using 5-channel PQK embeddings. Type~1 outperforms Type~2 but both are exceeding the classical baseline.}
\end{table}
\item[2.] \textbf{Training Dynamics:} \
The convergence patterns reveal that Type~1 PQK-augmented models converge substantially faster. The 20-channel variant surpasses 90\% validation accuracy in fewer than 15 epochs, while the 5-channel Type~2 model often stagnates below 90\% for over 80 epochs. This shows that richer and more structured quantum embeddings lead to more efficient learning.

\item[3.] \textbf{Generalization and Overfitting:} \
Classical CNN shows a mild overfitting gap (~2\%), which is preserved in the Type~1 hybrid. However, PQK-only models, despite achieving near-perfect training scores, generalize poorly (67.5\% validation), highlighting the necessity of classical features. Type~2 models sometimes underfit, particularly in low-dimension settings.

\item[4.] \textbf{Quantum Circuit Feature Behavior:}  We analyze the entropy of photon detection patterns. Type~1 PQK circuits exhibited low entropy, suggesting structured interference. Type~2 showed entropy near 0.999, indicative of noisy, uncorrelated outputs. Visual inspection of quantum feature maps also showed richer diversity in Type~1. The mode correlation matrices aligned with this analysis, as Type~1 showed more significant off-diagonal interactions.



% ————— end of inserted plots —————


\item[5.] \textbf{Key Takeaways:} 
\begin{itemize}
  \item Type~1 encoding leads to stronger, structured features and higher accuracy.
  \item Higher quantum output dimensionality (20 vs. 5 channels) significantly improves learning.
  \item Type~2’s high entropy output lacks structure and degrades model performance.
  \item PQK-only networks overfit, proving that classical features are indispensable.
  \item Circuit properties such as entanglement and interference correlate with model success.
\end{itemize}

\item[6.] \textbf{Conclusion:} \
This analysis confirms that photonic quantum kernels can benefit classical models when used in a hybrid framework. Effectiveness depends heavily on the encoding scheme and feature dimensionality. Well-designed quantum circuits — particularly Type~1 encoding with sufficient entanglement — yield useful features that complement classical learning. These insights open the path to extending PQK-based models to more complex datasets and deeper architectures.

\end{itemize}

==> participants_sections/Qubiteers/proposal_old.tex <==
% ----------------------------
% Model Proposal Section
% ----------------------------

We propose a hybrid quantum-classical image classification model that leverages a \emph{Photonic Quantum Kernel} (PQK) alongside a classical CNN. The PQK acts like a convolutional kernel by processing each $2\times2$ image patch through a photonic interferometer. Pixel intensities are normalized and encoded as phase shifts, modulating the path of single photons through beam splitter layers. The output detection pattern becomes the quantum feature vector for that patch. The full image is scanned with stride 2, producing a feature map composed of 5 or 20 channels per patch. Boson sampling is implemented using Perceval (a software development kit for programming photonic quantum computers). This method leverages quantum interference in high-dimensional Hilbert spaces to encode complex local correlations that classical kernels may miss. Here, 2 types of PQK are proposed: Type~1 PQK and Type~2 PQK.

%Our study compares three architectures: (1) a baseline CNN, (2) a hybrid CNN with Type~1 PQK, (3) a hybrid CNN with Type~2 PQK and (4) a hybrid model with CNN and trainable Type~2 PQK. 
%We evaluated the performance of the MNIST dataset in terms of accuracy, convergence speed, and generalization.

\begin{itemize}

  \item[1.] \textbf{Classical CNN Baseline:} \\ 
  We use a conventional CNN with two convolutional layers (32 and 64 filters) each followed by ReLU activation and $2\times2$ max-pooling, followed by two dense layers ($3136\to128\to10$). This model contains around $4.2\times10^5$ trainable parameters. It is trained using the Adam optimizer (learning rate $10^{-3}$) and cross-entropy loss. The model achieves 97.6\% validation accuracy and 99.6\% training accuracy on the reduced MNIST dataset of batch-size 160. This architecture converges within 10–20 epochs and serves as a reliable baseline to compare quantum enhancements. The circuit defined in the baseline operates on 20 hard-coded modes without any kernel-based encoding. It comprises of 7 layers, each with staggered beam splitters ($r \in [0.4, 0.6]$) and random phase shifters ($\phi \in [0, 2\pi]$).

  \item[2.] \textbf{Photonic Quantum Kernel (PQK):} \\ 
  The PQK acts like a convolutional kernel by processing each $2\times2$ image patch through a photonic interferometer. Pixel intensities are normalized and encoded as phase shifts, modulating the path of single photons through beam splitter layers. The output detection pattern becomes the quantum feature vector for that patch. The full image is scanned with stride 2, producing a feature map composed of 5 or 20 channels per patch. Boson sampling is implemented using Perceval (a software development kit for programming photonic quantum computers). This method leverages quantum interference in high-dimensional Hilbert spaces to encode complex local correlations that classical kernels may miss.

  \item[3.] \textbf{Encoding Strategies:}
  \begin{itemize}
    \item \textbf{Type~1 (Naive Encoding):} Each pixel in the $2\times2$ kernel is assigned to a separate photonic mode. All four modes are populated simultaneously, enabling full interference and dense entanglement. This one-shot encoding captures holistic correlations within the patch. The example circuit for a $3\times3$ kernel with depth $1$ of interference can be seen in  figure~\ref{fig:type1_circuit}.
    \item \textbf{Type~2 (Compressed Encoding):} Two pixels are encoded first, followed by beam splitter layers. Then the remaining two pixels are encoded. This staggered process uses fewer initial modes ($\left\lceil kernel\_size^2/2 \right\rceil$) and promotes preferential mixing of information. It potentially captures different aspects of the data structure as compared to Type~1. The example circuit for a $3\times3$ kernel with depth $2$ of interference can be seen in Figure~\ref{fig:type2_circuit}. The circuit in the figure is an example of static/non-trainable kernel where as the depth increases, the degree of rotation of each of the modes decreases in powers of $2$. This depth-wise rotation was implemented to see the effect of decreasing interactivity among the modes.
    \item \textbf{Type~2 Trainable Kernel} Extending the idea of Type~2 encoding kernel, we also implement a circuit, where after the kernel pixel values are encoded, the interference is controlled by trainable parameters. We use Quandela's Merlin framework and distributing the input image into patches to accelerate convolution operations and the training of the parameters in the kernel circuit. An example circuit for this trainable kernel can be seen in Figure~\ref{fig:type2_circuit_trainable}.
  \end{itemize}

\begin{figure}[h!]
\centering
\includegraphics[width=0.75\columnwidth]{figures/qubiteers/PQK Kernel Type 1.png}
\caption{Photonic quantum kernel circuit: Type~1 (simultaneous) encoding. \emph{(Placeholder)}}
\label{fig:type1_circuit}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{figures/qubiteers/PQK Kernel Type 2 cropped.png}
\caption{Photonic quantum kernel circuit: Type~2 (delayed) encoding. \emph{(Placeholder)}}
\label{fig:type2_circuit}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{figures/qubiteers/PQK Kernel Type 2 trainable.png}
\caption{Photonic quantum kernel circuit: Type~2 (delayed) encoding. \emph{(Placeholder)}}
\label{fig:type2_circuit_trainable}
\end{figure}

  \item[4.] \textbf{Hybrid PQK-CNN Architecture:} \\ 
  We construct a dual-path network with parallel quantum and classical branches:
  \begin{itemize}
    \item \textbf{Classical Branch:} Applies standard CNN operations on the raw $28\times28$ grayscale image, extracting spatial features using convolution, pooling, and ReLU. We have two layers of classical CNN. The first layer has a kernel size of $3\times3$ with a padding of $0$ and outputs $16$ filters. The input for this layer is (1, 28, 28) and the output is of the shape (16, 26, 26). The second layer has the kernel of size $5\times5$, again with padding $0$ and outputs $32$ filters. For this layer, the input is (16, 26, 26) and output is (32, 22, 22).
    \item \textbf{Quantum Branch (Non-Trainable):} Applies PQK-based convolutions with stride 2 over $2\times2$ patches. Each patch yields a 5 or 20 channel feature vector, aggregated into a $14\times14\times N$ quantum feature map. These are passed through one or two small convolutional layers with ReLU to enhance representation. The PQK convolution was accelerated with the help of multi-threading and multiple sessions managed with the help of Scaleway. The input images are pre-processed with the help of these non-trainable kernel convolutions and then given as input to the classical post-NN to get the final class label.
    \item \textbf{Quantum Branch (Trainable Kernel):} We also implement a parallel-branched model where the quantum branch performs the convolution operations of the trainable Type~2 PQK. In this case, the original input images cannot be pre-processed and stored and used later when required. Since the kernel circuit in this case contains trainable parameters, the PQK convolutions need to be applied every time the model is called. To implement this, a custom convolution class is implemented which converts the kernel circuit into a Merlin layer and implements this circuit on all the patches generated for the input image for that convolution layer. Merlin helps to accelerate this process by using a GPU on the image patches.
    \item \textbf{Fusion:} Classical and quantum outputs are concatenated channel-wise. The combined tensor is flattened and passed through a dense network (128 hidden units, 10 output classes). This fusion allows the network to exploit both standard pixel features and high-order quantum-derived patterns. In a slightly different setup, the outputs from the final classical and PQK layers are concatenated to form tensors of shape (64, 22, 22). This is passed through a classical CNN layer of kernel size $3\times3$ with a padding of $1$. The output from this layer is (32, 22, 22). This tensor is then flattened and then passed through a classical feedforward neural network (FNN) (15488 $\rightarrow$ 512 $\rightarrow$ 64 $\rightarrow$ 10). This setup can be seen in Figure~\ref{fig:hybrid_arch__parallel_type2_trainable}.
  \end{itemize}
  Additionally, we experiment with a PQK-only model to evaluate the independent utility of quantum embeddings.

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\columnwidth]{figures/qubiteers/PQK-CNN combined model 2.png}
\caption{Hybrid CNN+PQK architecture. Classical and quantum branches process the image in parallel. Final predictions are based on merged features. \emph{(Placeholder)}}
\label{fig:hybrid_arch__parallel_type2_trainable}
\end{figure}

  \item[5.] \textbf{Training Setup:} \\ 
  All models are trained on the MNIST dataset consisting of 60,000 training and 10,000 test images. We reserve 10\% of the training set for validation. Training is performed with mini-batches of size 32, using the Adam optimizer with a learning rate of $10^{-3}$ and cross-entropy loss. The baseline CNN converges within 20 epochs. Hybrid models train up to 50 epochs with early stopping. For 5-channel PQK embeddings, convergence may require up to 100 epochs due to reduced input dimensionality.
  
  The PQK circuits are non-trainable and simulated using Quandela’s Perceval library. To mitigate local resource constraints, we offload quantum computations to Scaleway's Quantum-as-a-Service platform. We use a 25-mode, 10-photon interferometer, where each image patch is processed into quantum features by encoding pixel intensities as phase shifts on photons. Parallel cloud jobs are deployed to process all 14 patch rows per image concurrently, yielding a $\sim14\times$ speedup. Only the classical CNN weights and classifier are updated via backpropagation, while PQK outputs remain fixed for a given input. This setup allows scalable training with realistic quantum constraints.

\end{itemize}

==> participants_sections/Qubiteers/supp_old.tex <==
We defined a slightly modified version of the Kronecker Delta to simplify the calculations for different arrangements of the Beam Splitters in our kernel circuits. We use the 0-indexed notation everywhere including indexing the modes and the rows and columns of the matrices. This new BS-delta ($\delta'_{jk}$) is $1$ if the wires indexed $j$ and $k$ are interacting through a BS. This delta can be defined as:
\begin{equation}
    \delta'_{jk} =
    \begin{cases}
        1 & \text{if } j\neq k\ \text{and}\ BS\ \text{present between wires $j$ and $k$} \\
        0 & \text{else}
    \end{cases}
\end{equation}

The matrix for a single layer of Beam Splitters (BS) for a circuit with $m$ modes can be represented as:

\begin{align} \label{eq:sup}
   \begin{bmatrix}
1 & \delta'_{01}\mathrm{i} & \delta'_{02}\mathrm{i} & \cdots & \delta'_{0(m-1)}\mathrm{i} \\
       \delta'_{10}\mathrm{i} & 1 & \cdots & \cdots & \delta'_{1(m-1)}\mathrm{i} \\
       \delta'_{20}\mathrm{i} & \cdots & 1 & \cdots & \delta'_{2(m-1)}\mathrm{i} \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        \delta'_{(m-1)0}\mathrm{i} & \cdots & \cdots & \cdots & 1
    \end{bmatrix}
    &= \mathbb{I}_{m\times m} + 
    \begin{bmatrix}
        \delta'_{00}\mathrm{i}^{\delta'_{00}} & \delta'_{01}\mathrm{i} & \cdots & \delta'_{0(m-1)}\mathrm{i} \\
        \delta'_{10}\mathrm{i} & \delta'_{11}\mathrm{i} & \cdots & \delta'_{1(m-1)}\mathrm{i} \\
        \vdots & \vdots & \ddots & \vdots \\
        \delta'_{(m-1)0}\mathrm{i} & \delta'_{(m-1)1}\mathrm{i} & \cdots & \delta'_{(m-1)(m-1)}\mathrm{i}
    \end{bmatrix} \nonumber \\
    &= \mathbb{I}_{m\times m} + 
    \begin{bmatrix}
        0 & \delta'_{01}\mathrm{i} & \cdots & \delta'_{0(m-1)}\mathrm{i} \\
        \delta'_{10}\mathrm{i} & 0 & \cdots & \delta'_{1(m-1)}\mathrm{i} \\
        \vdots & \vdots & \ddots & \vdots \\
        \delta'_{(m-1)0}\mathrm{i} & \delta'_{(m-1)1}\mathrm{i} & \cdots & 0
    \end{bmatrix}
\end{align}


with $j$ being the index of the rows and $k$ the index of the columns of the matrix. $i$ represents the complex number iota. This comes from the matrix for the default BS used by Perceval. Equation~\ref{eq:sup} is unitary due to the fundamental nature of beam splitter operations, which are lossless and energy-preserving. As an example, the matrix for the first and second layers of interference in a $3\times3$ Type~1 kernel circuit, such as in~\ref{fig:type1_circuit}, can be expressed, respectively, as:

\begin{equation}
    M_{L1} = 
    \begin{bmatrix}
        1 & i & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        i & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 1 & i & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & i & 1 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & i & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & i & 1 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 & 1 & i & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 & i & 1 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
    \end{bmatrix}_{9\times9}
    \quad
    M_{L2} = 
    \begin{bmatrix}
        1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 1 & i & 0 & 0 & 0 & 0 & 0 & 0 \\
        0 & i & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 & i & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & i & 1 & 0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 1 & i & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & i & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & i \\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & i & 1 \\
    \end{bmatrix}_{9\times9}
\end{equation}

Our supplementary ablation studies targeted the core components of the PQK-enhanced architecture to isolate their impact on classification performance.

In both our Type~1 and Type~2 kernel circuits, we use this brickwall-type design of BSs, multiple times. For such an arrangement, the matrices for layers 1 and 2 can be multiplied as:

\begin{equation}
    a_{xy} = \sum_{n=0}^{m-1} M_{L2}[x, n]\cdot M_{L1}[n, y]\ ;\ x, y: 0 \rightarrow m-1
\end{equation}

where $a_{xy}$ is the element at row $x$ and column $y$ and $M_{L1}[x, n]$ is the element at row $x$ and column $n$ in matrix $M_{L1}$. This can be re-written as:

\begin{equation}
    a_{xy} = \sum_{n=0}^{m-1} (\delta_{xn} + \delta^{2'}_{xn}i)\cdot (\delta_{ny} + \delta^{1'}_{ny}i)
    \label{eq:bs_single_layer}
\end{equation}

Here, $\delta^{1'}$ is the $\delta'$ operator for the first layer of the BS arrangement in the 2-layer bricklayer arrangement. Similarly, $\delta^{2'}$ is the $\delta'$ operator for the second layer.

\begin{equation}
    a_{xy} = \sum_{n=0}^{m-1} (\delta_{xn}\cdot\delta_{ny} + \delta_{xn}\cdot\delta^{1'}_{ny}i + \delta_{ny}\cdot\delta^{2'}_{xn}i - \delta^{2'}_{nx}\cdot\delta^{1'}_{yn})
\end{equation}

% Following the definitions of the Kronecker Delta and BS Delta (defined before), we can say that:
% \begin{equation}
%     \delta_{xn}\cdot\delta'_{ny} = \delta'_{xy}
% \end{equation}
% This is because, the left hand side (LHS) will be $1$ if and only if $\delta_{xn}$ is $1$, when $x$ = $n$ and $\delta'_{ny}$ is $1$, when $n$ $\neq$ $y$ and modes $n$ and $y$ interact through a BS. This can be seen as $x$ $\neq$ $y$ and modes $x$ and $y$ interact through a BS. This becomes $\delta'_{xy}$ on the right hand side.

\begin{equation}
    a_{xy} = \delta_{xy} + \delta_{xx}\cdot\delta^{1'}_{xy}i + \delta_{yy}\cdot\delta^{2'}_{xy}i - \sum_{n=0}^{m-1} (\delta^{2'}_{nx}\cdot\delta^{1'}_{yn})
\end{equation}
\begin{equation}
    a_{xy} = \delta_{xy} + \delta^{1'}_{xy}i + \delta^{2'}_{xy}i - \sum_{n=0}^{m-1} (\delta^{2'}_{nx}\cdot\delta^{1'}_{yn})
\end{equation}

We can expand this equation into a piece-wise definition:

\begin{equation}
    a_{xy} = \delta_{xy} + 
    \underbrace{
    \begin{cases} 
        i & \text{if } \delta^{1'}_{xy}=1 \\ 
        0 & \text{if } \delta^{1'}_{xy}=0 
    \end{cases} 
    + 
    \begin{cases} 
        i & \text{if } \delta^{2'}_{xy}=1 \\ 
        0 & \text{if } \delta^{2'}_{xy}=0 
    \end{cases}}_{\in \{0, i\}}
     - \sum_{n=0}^{m-1} (\delta^{2'}_{nx}\cdot\delta^{1'}_{yn})
    % + \sum_{n=0}^{m-1} 
    % \begin{cases} 
    %     -1 & \text{if } \delta^{2'}_{xn}=1 \text{ and } \delta^{1'}_{ny}=1 \\ 
    %     0 & \text{else} 
    % \end{cases}
\end{equation}

The second and third terms can be reduced to either $0$ or $i$. This is because if $\delta^{1'}_{xy}$ is $1$, then $\delta^{2'}_{xy}$ will be $0$. This comes from the bricklayer arrangement that no two consecutive modes interact through a BS in both the layers. However, there can be a case where both these terms are $0$, when $x$ and $y$ are not consecutive modes or $x$ = $y$. The equation now becomes:

\begin{equation}
    a_{xy} = \delta_{xy} + \delta'_{xy}i - \sum_{n=0}^{m-1} (\delta^{2'}_{nx}\cdot\delta^{1'}_{yn})
\end{equation}

The summation in the third term of the equation can be expanded by considering the inner term. This term is non-zero if both $\delta^{2'}_{nx}$ and $\delta^{1'}_{ny}$ are non-zero. This implies that there are BSs present between modes $x$ and $n$ in the first layer and between $y$ and $n$ in the second layer. If such an $n$ exists, the term becomes $-1$ and is $0$ in all other cases. Expanding on the case when the term is non-zero, it is only possible if the indices $x$, $n$ and $y$ are consecutive modes with $x < n < y$ or $y < n < x$ and $x$ and $y$ are at odd-index and even-index mode respectively. In all other cases, the term is $0$. The equation can be expanded as:

\begin{equation}
    a_{xy} = \delta_{xy} + \delta'_{xy}i
    - \sum_{n=0}^{m-1} 
    \begin{cases} 
        1 & \text{if } \delta^{2'}_{xn}=1 \text{ and } \delta^{1'}_{ny}=1 \\ 
        0 & \text{else}
    \end{cases}
\end{equation}

\begin{equation}
    a_{xy} = \delta_{xy} + \delta'_{xy}i
    - 
    \begin{cases} 
        1 & \text{if } \delta_{(x\%2)(y>x)} \text{ and } \lvert x - y\rvert = 2 \\ 
        0 & \text{else}
    \end{cases}
\end{equation}

We can re-write this element assignment as:

\begin{equation}
    a_{xy} = 
    \begin{cases}
        1 & \text{if } \lvert x - y\rvert = 0 \\
        i & \text{if } \lvert x - y\rvert = 1 \\
        -\delta_{(x\%2)(y>x)} & \text{if } \lvert x - y\rvert = 2 \\
        0 & \text{else}
    \end{cases}
    \label{eq:bs_brick}
\end{equation}

% On expanding the summation, the equation can be expanded as:

% \begin{equation}
%     a_{xy} = \delta_{xy} + \delta'_{xy}i
%     - 
%     \begin{cases} 
%         1 & \text{if } \lvert x - y\rvert = 2 \\ 
%         0 & \text{else }
%     \end{cases}
%     \ ;\ x, y: 0 \rightarrow m-1
% \end{equation}

Following this equation, we can form the matrix for a $9$-mode Type~1 kernel (figure~\ref{fig:type1_circuit}) as:

\begin{equation}
    M_{L21} = 
    \begin{bmatrix}
        1 & i & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        i & 1 & i & -1 & 0 & 0 & 0 & 0 & 0 \\
        -1 & i & 1 & i & 0 & 0 & 0 & 0 & 0 \\
        0 & 0 & i & 1 & i & -1 & 0 & 0 & 0 \\
        0 & 0 & -1 & i & 1 & i & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 & i & 1 & i & -1 & 0 \\
        0 & 0 & 0 & 0 & -1 & i & 1 & i & 0 \\
        0 & 0 & 0 & 0 & 0 & 0 & i & 1 & i \\
        0 & 0 & 0 & 0 & 0 & 0 & -1 & i & 1
    \end{bmatrix}_{9\times9}
\end{equation}

It can be confirmed that the matrix $M_{l1l2}$ is equal to the matrix obtained after multiplying the matrices $M_{L2}$ and $M_{L1}$. The element assignment rules from equations~\ref{eq:bs_single_layer} and~\ref{eq:bs_brick}, help us in doing the calculations for both types of kernel circuits.

The matrices for patch encoding and assignment of trainable parameters done using Phase Shifters (PS) can be written as:

\begin{equation}
    U_{enc} = 
    \begin{bmatrix}
        e^{ip_0} & 0 & \dots & 0 \\
        0 & e^{ip_1} & \dots & 0 \\
        0 & 0 & \dots & 0 \\
        0 & 0 & \dots & e^{ip_{m-1}}
    \end{bmatrix}_{m\times m}
    \quad
    U_{trainable} = 
    \begin{bmatrix}
        e^{i\theta_0} & 0 & \dots & 0 \\
        0 & e^{i\theta_1} & \dots & 0 \\
        0 & 0 & \dots & 0 \\
        0 & 0 & \dots & e^{i\theta_{m-1}}
    \end{bmatrix}_{m\times m}
\end{equation}

% \begin{equation}
%     a_{xy} = \sum_{n=0}^{8} \delta'_{xn}\cdot\delta'_{ny}\cdot i^{\delta'_{xn}}\cdot i^{\delta'_{ny}}
%            = \sum_{n=0}^{8} \delta'_{xy}\cdot i^{\delta'_{xn}+\delta'_{ny}}
% \end{equation}

% Here, $x$ and $y$ are either equal or unequal. In that case, $\delta'_{xy}$ and $\delta_{xy}$ will be $0$ respectively. Therefore the term becomes:

% \begin{equation}
%     a_{xy} = 9\delta_{xy} + \delta'_{xy}\sum_{n=0}^{8} (i^{\delta'_{xn}+\delta'_{ny}})
% \end{equation}

% The full diagonal phase-shifting operation applied to the \(m \) modes can then be written as the product of patch-encoding and trainable parameter matrices:

% \begin{equation}
%     U_{\phi} = U_{enc} \cdot U_{trainable} = 
%     \begin{bmatrix}
%         e^{i(p_0 + \theta_0)} & 0 & \dots & 0 \\
%         0 & e^{i(p_1 + \theta_1)} & \dots & 0 \\
%         0 & 0 & \dots & 0 \\
%         0 & 0 & \dots & e^{i(p_{m-1} +\theta_{m-1})}
%     \end{bmatrix}_{m\times m}
% \end{equation}


==> quandela_sections/experiments.tex <==
\label{sec:experiments}
This section presents the results of the numerical experiments conducted on the models described in Section~\ref{sec:models}. Most of the models were implemented using quantum simulators, both ideal (noise-free) and noisy. Additionally, several experiments were executed on real photonic quantum processing units (QPUs) via Quandela’s cloud platform~\cite{quandela_cloud}. Many simulations also leveraged high-performance graphics processing units (GPUs) through Scaleway’s Quantum-as-a-Service platform~\cite{scaleway}, enabling large-scale quantum simulations. All quantum models are evaluated against classical baseline models, with comparisons made in terms of training and testing accuracy, number of trainable parameters, and computational cost measured in floating-point operations per second (FLOPS).
